Error-estimate-based Adaptive Integration For Immersed Isogeometric Analysis

The Finite Cell Method (FCM) together with Isogeometric analysis (IGA) has been applied successfully in various problems in solid mechanics, in image-based analysis, fluid-structure interaction and in many other applications. A challenging aspect of the isogeometric finite cell method is the integration of cut cells. In particular in three-dimensional simulations the computational effort associated with integration can be the critical component of a simulation. A myriad of integration strategies has been proposed over the past years to ameliorate the difficulties associated with integration, but a general optimal integration framework that suits a broad class of engineering problems is not yet available. In this contribution we provide a thorough investigation of the accuracy and computational effort of the octree integration scheme. We quantify the contribution of the integration error using the theoretical basis provided by Strang's first lemma. Based on this study we propose an error-estimate-based adaptive integration procedure for immersed isogeometric analysis. Additionally, we present a detailed numerical investigation of the proposed optimal integration algorithm and its application to immersed isogeometric analysis using two- and three-dimensional linear elasticity problems.

==> Chapters/operatorconstants.tex <==
\section{Operator-dependence of the cut cell integration errors} \label{sec:operatorconstants}
The cut cell integration errors $e_K^b$ and $e_K^a$ in equation \eqref{eq:integrationerrorsindependent} depend on the operators $b^h$ and $a^h$, respectively. Both these operator-dependent errors are bound by the operator-independent cut cell integration error $e_K^p$ in equation \eqref{eq:polyerror}. The constants $\mathscr{C}_K^b$ and $\mathscr{C}_K^a$ in \eqref{eq:integrationerrorsindependent} are dependent on the considered operators.

To illustrate how these constants depend on the operators, we consider the linear operator $b^h$ with integrand $B^h_\Omega$ as an element of the class of linear operators $\mathcal{L}(V_K^h, P_K)$. An operator in this class maps the localized test space onto a normed space $P_K:K \rightarrow \mathbb{R}$, which is chosen such that $B^h_\Omega \circ V^h_K \subseteq P_K$. By defining the operator norm
\begin{align}
  \| B^h_\Omega \|_{\mathcal{L}(V^h_K,P_K)} := \sup \limits_{v^h_K \in V^h_K} \frac{ \| B^h_\Omega ( v^h_K  ) \|_{P_K}  }{\| v_K^h \|_{V^h_K}},
\label{eq:operatornorm}
\end{align}
the integration error for $b^h$ can be expressed as
	\begin{align}
	e_K^{b} &=\sup_{v^h_K \in {V}^h_K} \frac{  \left|\int_{K} {B_\Omega^h}(v^h_K)\,{\rm d}V -  \sum \limits_{l=1}^{l_K} \omega^l_K B_\Omega^h(v^h_K(\boldsymbol{x}_K^l) ) \right| }{ \left\| v^h_K \right\|_{V_K^h}} \nonumber \\
	&\leq   \| B_\Omega^h  \|_{\mathcal{L}(V_K^h,P_K)} \sup_{v^h_K \in {V}^h_K}{\frac{  \left|\int_{K} B_\Omega^h(v^h_K)\,{\rm d}V -  \sum \limits_{l=1}^{l_K} \omega^l_K {B_\Omega^h}(v^h_K(\boldsymbol{x}_K^l))\right| }{ \| B_\Omega^h(v^h_K) \|_{P_K} } } \nonumber \\
	&\leq    \| B_\Omega^h  \|_{\mathcal{L}(V^h_K,P_K)} \sup_{p_K \in  B_\Omega^h\circ V_K^h}{\frac{  \left|\int_{K} p_K(\boldsymbol{x}_K) \,{\rm d}V -  \sum \limits_{l=1}^{l_K} \omega^l_K {p_K}(\boldsymbol{x}_K^l)\right| }{ \| p_K \|_{P_K} } } \nonumber \\
	&\leq    \| B_\Omega^h  \|_{\mathcal{L}(V_K^h,P_K)} \, e_K^{p} \label{eq:elem_interrorFPoly}
	\end{align}
with the operator-independent element integration error defined as \eqref{eq:polyerror}. From \eqref{eq:integrationerrorsindependent} it directly follows that:
\begin{align}
\mathscr{C}_K^b =  \| B_\Omega^h  \|_{\mathcal{L}(V_K^h,P_K)}
\end{align}
The constant $\mathscr{C}_K^a$ can similarly be related to the operator $A^h_\Omega$.


